TableMaster: A Recipe to Advance Table Understanding with Language Models

Tables serve as a fundamental format for representing structured relational data. While current language models (LMs) excel at many text-based tasks, they still face challenges in table understanding due to the complex characteristics of tabular data, such as their structured nature. In this paper, we aim to enhance LMs for improved table understanding. We identify four key challenges: 1) difficulty in locating target data, 2) deficiency in table semantics, 3) numerical inaccuracies in textual reasoning, and 4) semantic inflexibility in symbolic reasoning. To address these issues, we propose TableMaster, a recipe and comprehensive framework that integrates multiple solutions to overcome these obstacles. TableMaster first extracts relevant table content and verbalizes it with enriched semantic context. Additionally, we introduce adaptive reasoning, a flexible approach that dynamically adjusts between textual and symbolic reasoning, tailoring the reasoning process to each query. Extensive analyses and experiments demonstrate our findings and the effectiveness of TableMaster. On the WikiTQ dataset, TableMaster achieves an accuracy of 78.13% using GPT-4o-mini, surpassing existing baselines. We hope this work will serve as a practical step toward more robust and reliable table understanding.

==> figures/challenge.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/sources/challenge.pdf}
    \caption{Experimental analysis of challenges in table understanding with language models. (a) Impact of table size on task difficulty. (b) Effect of verbalized tables with enriched semantic context. (c) Performance comparison of different reasoning methods on calculation-required versus non-calculation questions. (d) Performance differences when processing normalized versus noisy tables.}
    \label{fig:challenge}
\end{figure*}

==> figures/overview.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/sources/overview.pdf}
    \caption{Overview of the challenges and proposed solutions in this work. Tabular data is inherently structured, dense, concise, and numerical. Based on these characteristics, we identify four key challenges. To address them, we propose four targeted solutions. The gray arrows between the characteristics and challenges represent the potential causes of these challenges stemming from specific characteristics. Each proposed solution corresponds to the challenge presented on the left in the same row. \method is a unified recipe developed based on these findings.}
    \label{fig:overview}
\end{figure}

==> figures/peek.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/sources/peek.pdf}
    \caption{test}
    \label{fig:peek}
\end{figure*}

==> figures/wikitq_row.tex <==
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\textwidth]{figures/sources/wikitq_row.pdf}
    \caption{test}
    \label{fig:wikitq_row}
\end{figure*}
